Learning Independent Object Motion from Unlabelled Stereoscopic Videos

We present a system for learning motion of independently moving objects from stereo videos. The only human annotation used in our system are 2D object bounding boxes which introduce the notion of objects to our system. Unlike prior learning based work which has focused on predicting dense pixel-wise optical flow field and/or a depth map for each image, we propose to predict object instance specific 3D scene flow maps and instance masks from which we are able to derive the motion direction and speed for each object instance. Our network takes the 3D geometry of the problem into account which allows it to correlate the input images. We present experiments evaluating the accuracy of our 3D flow vectors, as well as depth maps and projected 2D optical flow where our jointly learned system outperforms earlier approaches trained for each task independently.

==> section/loss_functions.tex <==
\begin{figure}[tb]
    \centering
    \includegraphics[width=1\linewidth]{Figure/sec3/depth_consistency.pdf} \\
 \vspace{-10pt}
    \caption{Illustration of our photometric and depth consistency losses. A pixel from image $I_{t}$ is unprojected at its ground truth (red) or predicted depth (blue) and subsequently transformed to the frame of $I_{t+1}$ using the ground truth ($F_{gt}$) or predicted flow ($F_{pred}$) and the camera transform $T_{t,t+1}$. The photometric consistency loss is derived from the photometric difference between $I_t$ warped into the frame of $I_{t+1}$ in the above manner. The depth consistency loss is computed by comparing the difference between nearness maps warped in the above manner. Note that using only photometric consistency would not resolve the ambiguity in the $z$ direction of the flow. }. 
    
    \label{fig:depth_consist}
\end{figure}



\section{Loss Functions for Flow and Depth}
\label{sec:losses}


In order to train our network we need suitable training data and loss functions. The difficulty is that scene flow ground truth is generally not something which is available for real data. The reason for this is that there is no easy way to measure even optical flow in the real world. Therefore common benchmarks generate the ground truth by either spraying an easily matchable pattern to the scene \cite{baker2011database} or by using human annotations \cite{Menze2015CVPR}. 

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{Figure/sec3/reprojection.pdf} \\
 \vspace{-10pt}
    \caption{Reprojection in dynamic scene. (a), (b) are two consecutive frames where the van is moving forward. (c) is the reprojection result by reprojecting the pixels from frame 1 to frame 0 using the GT depth. (d) is the difference between (a) and (c). (e) is the reprojection result by reprojecting the pixels from frame 1 to frame 0 using the GT depth and 3d flow. (f) is the difference between (a) and (e). With the consideration of object movements, the reprojection result is more consistent and thus the resulting loss will provide better supervision signal in the training process.}
    %\vspace{-12pt}
    \label{fig:reprojection}
\end{figure}


\subsection{Photometric Consistency Loss}

If no ground truth flow or depth is given we are still able to use the images themselves as supervision and hence train our network in a self-supervised manner by exploiting the photometric consistency of multiple views of the same scene. The basic principle is that given a pixel in image $I_\mathrm{ref}$ we can use the scene flow and depth to warp it into another view $I_i$ and compare the similarity of the image pixels. With bilinear interpolation a gradient is computed which serves as training signal for the depth and the flow \cite{garg2016unsupervised}.

In order to compute the photometric loss we warp image $I_\mathrm{i \neq \mathrm{ref}}$ using the knowledge about the relative camera motion, scene flow $F_\mathrm{ref}$ and depth $D_\mathrm{ref}$ to the reference view, which leads to a warped image $\hat{I}_i$. If ground truth depth is available we can use the ground truth depth for the warp. In the case where no ground truth depth is available both the scence flow and the depth are predictions. Additionally, we can also use the depth and the flow to predict an occlusion/disocclusion  mask $\hat{M}_i$ which is $0$ is a pixel is occluded and $1$ otherwise. The photmetric loss is then defined as

\begin{equation}
    \mathcal{L}_\mathrm{photo} = \lambda_p \left\| \operatorname{vec}\left(\hat{M}_i \odot (I_\mathrm{ref} - \hat{I}_i)\right) \right\|_1.
\end{equation}



%~\cite{zhou2017unsupervised} assumes the scene is static. For dynamic scene, object motion needs to be considered. Fig.~\ref{fig:reprojection}


\subsection{Depth Consistency Loss}



Using the photometric consistency loss alone can be an insufficient training signal. The reason is that along a viewing ray multiple photo consistent solutions are possible, as shown in Fig.~\ref{fig:depth_consist}. Therefore we propose to additionally use a consistency loss on the depth which constrains the flow further. The depth can either be predicted by the network or come from ground truth measurements.

Analogously to the photometric loss the geometric loss is defined based on warping the depth. The geometric loss is then defined as

\begin{equation}
    \mathcal{L}_\mathrm{geo} = \lambda_g \left\| \operatorname{vec}\left(\hat{M}_i \odot (D_\mathrm{ref} - \hat{D}_i)\right) \right\|_1.
\end{equation}

 
